A separate way to measure rate of return

Net profit is sometimes found from data for net operating surplus. We propose a way to find it from data for consumption, pay and market-value capital, and concomitantly to reveal the factor shares in consumption.

==> tables/old_tables/old_fgr_table.tex <==
\begin{table}[pos = H]%
% \vspace*{-2cm}%
\caption{Average \(f(K)\), \(g(K)\) and \(r(K)\) in all countries, in descending order of net income per capita(\%).}%
\makebox[\textwidth][c]{
{\centering 
\begin{tabular}{lllll}
\toprule
Country & Period & $f(K)$ & $g(K)$ & $r(K)$ \\
\midrule
Luxembourg & 1996 - 2018 & 1.93 & 4.50 & 6.43\\
Switzerland & 1995 - 2019 & 0.88 & 3.70 & 4.58\\
Norway & 1981 - 2020 & 3.55 & 5.64 & 9.19\\
USA & 1970 - 2018 & 4.44 & 3.56 & 7.99\\
Denmark & 1996 - 2020 & 2.16 & 5.42 & 7.59\\
\addlinespace
Netherlands & 1996 - 2019 & 2.42 & 3.35 & 5.77\\
Austria & 1996 - 2019 & 2.67 & 2.59 & 5.27\\
Sweden & 1950 - 2020 & 2.59 & 4.25 & 6.84\\
Saudi Arabia & 2002 - 2009 & 10.88 & 5.73 & 16.61\\
Iceland & 2000 - 2014 & 3.27 & 3.39 & 6.67\\
\addlinespace
Belgium & 1996 - 2019 & 1.54 & 2.80 & 4.33\\
Germany & 1990 - 2020 & 3.53 & 3.11 & 6.64\\
New Zealand & 1999 - 2017 & 2.46 & 5.65 & 8.12\\
France & 1950 - 2019 & 2.39 & 4.28 & 6.67\\
Ireland & 1996 - 2019 & 2.51 & 5.61 & 8.12\\
\addlinespace
Finland & 1996 - 2020 & 3.79 & 4.06 & 7.85\\
Australia & 1960 - 2019 & 2.40 & 4.45 & 6.85\\
Canada & 1972 - 2020 & 2.82 & 4.45 & 7.27\\
Cyprus & 1996 - 2019 & 6.93 & 4.94 & 11.87\\
Israel & 2000 - 2019 & 13.93 & 8.75 & 22.68\\
\addlinespace
Malta & 1996 - 2019 & 2.50 & 4.01 & 6.51\\
UK & 1970 - 2019 & 5.11 & 3.00 & 8.11\\
Spain & 1995 - 2019 & 2.72 & 3.57 & 6.28\\
Japan & 1980 - 2017 & 2.28 & 2.81 & 5.09\\
Aruba & 1996 - 2000 & 26.05 & 28.80 & 54.85\\
\addlinespace
Venezuela & 1997 - 2007 & 32.48 & 6.69 & 39.17\\
Slovenia & 1996 - 2019 & 1.10 & 1.72 & 2.82\\
Lithuania & 1996 - 2019 & 8.20 & 4.49 & 12.69\\
Czech Rep. & 1994 - 2019 & 2.67 & 1.07 & 3.74\\
Italy & 1980 - 2020 & 4.89 & 2.84 & 7.73\\
\addlinespace
Estonia & 1996 - 2019 & 2.98 & 4.29 & 7.26\\
Poland & 1996 - 2019 & 10.72 & 5.86 & 16.58\\
Hungary & 1996 - 2019 & 2.51 & 3.13 & 5.63\\
Portugal & 1996 - 2020 & 2.77 & 2.54 & 5.32\\
\bottomrule
\end{tabular}
}

\centering{
\begin{tabular}{lllll}
\toprule
Country & Period & $f(K)$ & $g(K)$ & $r(K)$ \\
\midrule
Slovakia & 1996 - 2020 & 5.40 & 4.15 & 9.55\\
Romania & 1996 - 2019 & 7.25 & 2.54 & 9.79\\
Greece & 1996 - 2019 & 26.10 & 0.63 & 26.73\\
Turkey & 2009 - 2017 & 28.14 & 7.20 & 35.34\\
Croatia & 1996 - 2019 & 12.42 & 4.24 & 16.65\\
\addlinespace
Latvia & 1996 - 2019 & 4.39 & 4.30 & 8.69\\
Russian Fed. & 2008 - 2018 & 2.82 & -1.44 & 1.38\\
Uruguay & 2012 - 2016 & 5.21 & 1.36 & 6.58\\
Kazakhstan & 1996 - 2019 & 4.95 & 6.79 & 11.74\\
Malaysia & 2006 - 2015 & 32.47 & 12.36 & 44.83\\
\addlinespace
Chile & 1996 - 2009 & 14.27 & 6.72 & 20.99\\
Costa Rica & 2012 - 2017 & 8.84 & 5.21 & 14.04\\
Bulgaria & 1996 - 2017 & 5.10 & -0.09 & 5.00\\
Mexico & 1996 - 2019 & 10.25 & 3.28 & 13.53\\
Domin. Rep. & 1996 - 2016 & 33.68 & 8.44 & 42.12\\
\addlinespace
Serbia & 1997 - 2019 & 30.08 & 9.62 & 39.70\\
Brazil & 1996 - 2018 & 8.97 & 4.44 & 13.42\\
Colombia & 1996 - 2019 & 39.15 & 8.19 & 47.34\\
Azerbaijan & 1996 - 2010 & 39.68 & 13.76 & 53.44\\
Iran & 1996 - 2018 & 21.32 & 6.93 & 28.25\\
\addlinespace
Peru & 2007 - 2019 & 8.79 & 6.44 & 15.22\\
Egypt & 1996 - 2015 & 88.06 & 14.11 & 102.17\\
Moldova & 1998 - 2019 & 20.51 & 4.15 & 24.66\\
Mongolia & 2005 - 2019 & 4.29 & 6.86 & 11.16\\
Botswana & 1996 - 2000 & 20.19 & 6.70 & 26.89\\
\addlinespace
Guatemala & 2001 - 2019 & 24.90 & 6.98 & 31.89\\
Uzbekistan & 2015 - 2017 & 4.53 & 6.99 & 11.52\\
Cabo Verde & 2007 - 2017 & 22.72 & 3.82 & 26.54\\
Nicaragua & 2006 - 2018 & 6.65 & 5.11 & 11.76\\
Honduras & 2000 - 2015 & 20.88 & 8.54 & 29.42\\
\addlinespace
Kyrgyzstan & 1996 - 2019 & 20.79 & 4.09 & 24.87\\
Cote d’Ivoire & 1996 - 2000 & 61.84 & 29.54 & 91.38\\
Senegal & 2014 - 2015 & 28.95 & 8.68 & 37.63\\
Niger & 1996 - 2019 & 67.46 & 11.87 & 79.32\\
\bottomrule
\end{tabular}
}
}
\label{tbl-fgr_table}
\end{table}


==> tables/old_tables/old_shares_tbl.tex <==
\begin{table}[pos = H]%
% \vspace*{-2cm}%
\caption{Labor and capital shares\(^a\) in consumption in 68 countries in descending order of income per capita(\%).}%
\makebox[\textwidth][c]{
{\centering 
\begin{tabular}{llll}
\toprule
Country & Period & Labor Share & Capital Share\\
\midrule
Luxembourg & 1996 - 2018 & 81.53 & 18.47\\
Switzerland & 1995 - 2019 & 94.07 & 5.93\\
Norway & 1981 - 2020 & 79.97 & 20.03\\
United States & 1970 - 2018 & 81.00 & 19.00\\
Denmark & 1996 - 2020 & 89.85 & 10.15\\
\addlinespace
Netherlands & 1996 - 2019 & 85.21 & 14.79\\
Austria & 1996 - 2019 & 84.68 & 15.32\\
Sweden & 1950 - 2020 & 90.37 & 9.63\\
Saudi Arabia & 2002 - 2009 & 49.80 & 50.20\\
Iceland & 2000 - 2014 & 83.21 & 16.79\\
\addlinespace
Belgium & 1996 - 2019 & 86.56 & 13.44\\
Germany & 1990 - 2020 & 82.79 & 17.21\\
New Zealand & 1999 - 2017 & 81.38 & 18.62\\
France & 1950 - 2019 & 89.54 & 10.46\\
Ireland & 1996 - 2019 & 85.70 & 14.30\\
\addlinespace
Finland & 1996 - 2020 & 81.46 & 18.54\\
Australia & 1960 - 2019 & 85.65 & 14.35\\
Canada & 1972 - 2020 & 89.07 & 10.93\\
Cyprus & 1996 - 2019 & 70.97 & 29.03\\
Israel & 2000 - 2019 & 71.10 & 28.90\\
\addlinespace
Malta & 1996 - 2019 & 85.52 & 14.48\\
UK & 1970 - 2019 & 73.17 & 26.83\\
Spain & 1995 - 2019 & 81.21 & 18.79\\
Japan & 1980 - 2017 & 83.49 & 16.51\\
Aruba & 1996 - 2000 & 89.90 & 10.10\\
\addlinespace
Venezuela & 1997 - 2007 & 70.97 & 29.03\\
Slovenia & 1996 - 2019 & 92.18 & 7.82\\
Lithuania & 1996 - 2019 & 65.61 & 34.39\\
Czech Rep. & 1994 - 2019 & 81.58 & 18.42\\
Italy & 1980 - 2020 & 73.81 & 26.19\\
\addlinespace
Estonia & 1996 - 2019 & 83.33 & 16.67\\
Poland & 1996 - 2019 & 79.39 & 20.61\\
Hungary & 1996 - 2019 & 85.79 & 14.21\\
Portugal & 1996 - 2020 & 77.11 & 22.89\\
\bottomrule
\end{tabular}
}

\centering{
\begin{tabular}{llll}
\toprule
Country & Period & Labor Share &Capital Share\\
\midrule
Slovakia & 1996 - 2020 & 73.14 & 26.86\\
Romania & 1996 - 2019 & 65.39 & 34.61\\
Greece & 1996 - 2019 & 67.18 & 32.82\\
Turkey & 2009 - 2017 & 65.03 & 34.97\\
Croatia & 1996 - 2019 & 88.42 & 11.58\\
\addlinespace
Latvia & 1996 - 2019 & 70.34 & 29.66\\
Russia & 2008 - 2018 & 83.98 & 16.02\\
Uruguay & 2012 - 2016 & 71.01 & 28.99\\
Kazakhstan & 1996 - 2019 & 76.92 & 23.08\\
Malaysia & 2006 - 2015 & 62.18 & 37.82\\
\addlinespace
Chile & 1996 - 2009 & 72.38 & 27.62\\
Costa Rica & 2012 - 2017 & 72.33 & 27.67\\
Bulgaria & 1996 - 2017 & 67.82 & 32.18\\
Mexico & 1996 - 2019 & 56.91 & 43.09\\
Domin. Rep. & 1996 - 2016 & 63.64 & 36.36\\
\addlinespace
Serbia & 1997 - 2019 & 71.66 & 28.34\\
Brazil & 1996 - 2018 & 70.99 & 29.01\\
Colombia & 1996 - 2019 & 64.40 & 35.60\\
Azerbaijan & 1996 - 2010 & 63.15 & 36.85\\
Iran & 1996 - 2018 & 74.00 & 26.00\\
\addlinespace
Peru & 2007 - 2019 & 68.15 & 31.85\\
Egypt & 1996 - 2015 & 51.09 & 48.91\\
Moldova & 1998 - 2019 & 67.91 & 32.09\\
Mongolia & 2005 - 2019 & 73.33 & 26.67\\
Botswana & 1996 - 2000 & 51.74 & 48.26\\
\addlinespace
Guatemala & 2001 - 2019 & 52.58 & 47.42\\
Uzbekistan & 2015 - 2017 & 74.63 & 25.37\\
Cape Verde & 2007 - 2017 & 78.99 & 21.01\\
Nicaragua & 2006 - 2018 & 66.02 & 33.98\\
Honduras & 2000 - 2015 & 67.63 & 32.37\\
\addlinespace
Kyrgyzstan & 1996 - 2019 & 64.66 & 35.34\\
Côte d’Ivoire & 1996 - 2000 & 76.68 & 23.32\\
Senegal & 2014 - 2015 & 68.10 & 31.90\\
Niger & 1996 - 2019 & 38.32 & 61.68\\
\bottomrule
\end{tabular}
}
}
\raggedright{\footnotesize \(^a\) Derived at \(\frac{\Pi}{C}\) and \(\frac{C-\Pi}{C}\) respectively.}
\label{tbl-shares_table}
\end{table}

